Large-Scale Mixed-Bandwidth Deep Neural Network Acoustic Modeling for Automatic Speech Recognition

In automatic speech recognition (ASR), wideband (WB) and narrowband (NB) speech signals with different sampling rates typically use separate acoustic models. Therefore mixed-bandwidth (MB) acoustic modeling has important practical values for ASR system deployment. In this paper, we extensively investigate large-scale MB deep neural network acoustic modeling for ASR using 1,150 hours of WB data and 2,300 hours of NB data. We study various MB strategies including downsampling, upsampling and bandwidth extension for MB acoustic modeling and evaluate their performance on 8 diverse WB and NB test sets from various application domains. To deal with the large amounts of training data, distributed training is carried out on multiple GPUs using synchronous data parallelism.

==> conclusion.tex <==
\section{Summary}
\label{sec:sum}

In this paper we have investigated MB acoustic modeling for ASR with large-scale WB and NB training data. Various mixing strategies through upsampling, downsampling and BWE are evaluated on diverse test sets.  A VGG-based discriminatively trained BWE approach is proposed and investigated for its effectiveness. 
